LocAgent: Graph-Guided LLM Agents for Code Localization

Code localization--identifying precisely where in a codebase changes need to be made--is a fundamental yet challenging task in software maintenance. Existing approaches struggle to efficiently navigate complex codebases when identifying relevant code sections. The challenge lies in bridging natural language problem descriptions with the appropriate code elements, often requiring reasoning across hierarchical structures and multiple dependencies. We introduce LocAgent, a framework that addresses code localization through graph-based representation. By parsing codebases into directed heterogeneous graphs, LocAgent creates a lightweight representation that captures code structures (files, classes, functions) and their dependencies (imports, invocations, inheritance), enabling LLM agents to effectively search and locate relevant entities through powerful multi-hop reasoning. Experimental results on real-world benchmarks demonstrate that our approach significantly enhances accuracy in code localization. Notably, our method with the fine-tuned Qwen-2.5-Coder-Instruct-32B model achieves comparable results to SOTA proprietary models at greatly reduced cost (approximately 86% reduction), reaching up to 92.7% accuracy on file-level localization while improving downstream GitHub issue resolution success rates by 12% for multiple attempts (Pass@10). Our code is available at https://github.com/gersteinlab/LocAgent.

==> data/api_detail.tex <==
\begin{table}[ht!]
\resizebox{\linewidth}{!}{
    \centering
    \begin{tabular}{l m{5cm}}
        \toprule
        \textbf{API Name} & \textbf{Description} \\
        \midrule
        \makecell[l]{\texttt{search\_entity(} \\ 
            \quad \texttt{entity\_names: List[str]} \\
            \texttt{)}} & Searches the codebase to retrieve the complete implementations of specified entities based on the provided entity names.  \\
        \midrule
        \makecell[l]{\texttt{explore\_structure(} \\ 
            \quad \texttt{start\_entities: List[str],} \\
            \quad \texttt{direction: str = 'downstream',} \\
            \quad \texttt{traversal\_depth: int = 2,} \\
            \quad \texttt{entity\_type\_filter: Optional[List[str]] = None,} \\
            \quad \texttt{dependency\_type\_filter: Optional[List[str]] = None} \\
        \texttt{)}} & Analyzes and displays the dependency structure around specified entities in a code graph. \\
        \midrule
        \makecell[l]{\texttt{search\_code\_snippets(} \\ 
            \quad \texttt{search\_terms: Optional[List[str]] = None,} \\
            \quad \texttt{line\_nums: Optional[List] = None,} \\
            \quad \texttt{file\_path\_or\_pattern: Optional[str] = "**/*.py"} \\
        \texttt{)}} & Searches the codebase to retrieve relevant code snippets based on given queries(terms or line numbers). \\        
        \bottomrule
    \end{tabular}
    }
    \caption{List of unified APIs provided by LocAgent for code search and exploration.}
    \label{tab:tool_list}
    \vspace{-5mm}
\end{table}

==> data/main_precision.tex <==
% \begin{table*}[ht!]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llccc ccc ccc}
%         \toprule
%         \multirow{2}{*}{Method} & \multirow{2}{*}{Localization LM} & \multicolumn{3}{c}{File (\%)} & \multicolumn{3}{c}{Module (\%)} & \multicolumn{3}{c}{Function (\%)} \\
%         \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%         & & P@1 & P@3 & P@5 & P@3 & P@5 & P@10 & P@3 & P@5 & P@10 \\
%         \midrule
%         Agentless & gpt-4o & 67.0 & 24.8 & 14.9 & 23.3 & 14.1 & 7.0 & 20.8 & 13.1 & 6.5 \\
%         openhands & gpt-4o & 61.0 & 23.8 & 14.6 & 20.9 & 12.9 & 6.6 & 18.0 & 11.3 & 5.7 \\
%         moatless & gpt-4o & 73.3 & 28.0 & 16.9 & 25.5 & 15.8 & 8.1 & 20.4 & 13.5 & 7.1 \\
%         Ours & gpt-4o & 66.3 & 25.9 & 15.6 & 22.9 & 14.5 & 7.3 & 19.2 & 12.7 & 6.8 \\
%         \midrule
%         Agentless & claude-3.5 & 72.0 & 26.4 & 15.9 & 24.1 & 14.6 & 7.3 & 22.9 & 13.9 & 6.9 \\
%         openhands & claude-3.5 & 75.7 & 29.9 & 18.0 & 28.4 & 17.6 & 8.9 & 25.5 & 16.5 & 8.5 \\
%         moatless & claude-3.5 & 72.0 & 28.4 & 17.1 & 26.6 & 16.2 & 8.1 & 22.9 & 15.4 & 7.7 \\
%         Ours & claude-3.5 & 76.0 & 29.9 & 18.3 & 27.6 & 17.6 & 8.8 & 24.8 & 16.4 & 8.7 \\
%         Ours(1) & claude-3.5 & 74.3 & 30.2 & 18.6 & 28.6 & 17.6 & 8.8 & 25.3 & 16.8 & 8.7 \\
%         \textbf{Ours(2)} & claude-3.5 & 76.3 & \textbf{30.7} & \textbf{18.8} & \textbf{29.0} & \textbf{18.3} & \textbf{9.2} & \textbf{25.7} & \textbf{16.8} & \textbf{9.0} \\
%         Ours(3) & claude-3.5 & 76.0 & 30.9 & 18.8 & 29.0 & 18.3 & 9.3 & 25.5 & 16.8 & 9.2 \\
%         Ours(5) & claude-3.5 & 76.3 & 30.2 & 19.1 & 29.3 & 18.5 & 9.5 & 26.4 & 17.0 & 9.2 \\
%         \midrule
%         Qwen2.5-Coder-3 & 2B-Instruct & 66.1 & 26.1 & 15.9 & 21.2 & 13.5 & 6.8 & 17.0 & 11.7 & 6.2 \\
%         Ours & fine-tuned Qwen2.5-Coder-3 & 76.3 & 30.0 & 18.1 & 27.5 & 17.7 & 8.9 & 24.4 & 16.5 & 8.6 \\
%         Qwen2.5-Coder-7 & B-Instruct & 44.0 & 18.8 & 11.4 & 14.1 & 8.9 & 4.5 & 9.7 & 6.3 & 3.2 \\
%         Ours & fine-tuned Qwen2.5-Coder-7 & 70.3 & 28.1 & 17.0 & 25.8 & 16.3 & 8.3 & 21.0 & 14.6 & 7.9 \\
%         \bottomrule
%     \end{tabular}
% }
%     \caption{Precision analysis of different localization methods at various granularities.}
%     \label{tab:precision_comparison}
% \end{table*}


\begin{table*}[!ht]
    \centering
    \small
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{l|ll ccc cc cc}
        \toprule
        \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Loc-Model}} & \multicolumn{3}{c}{\textbf{File} (\%)} & \multicolumn{2}{c}{\textbf{Module} (\%)} & \multicolumn{2}{c}{\textbf{Function} (\%)}\\
        \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
         & & & \textbf{NDCG@1} & \textbf{NDCG@3} & \textbf{NDCG@5} & \textbf{NDCG@5} & \textbf{NDCG@10} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
        \midrule
        \midrule
        \multirow{5}{*}{Embedding-Based} 
            & \multicolumn{2}{l}{BM25~\cite{robertson2009probabilistic}} & 38.69	&46.5	&50.61	&37.31	&39.86	&26.15	&27.92 \\
            & \multicolumn{2}{l}{E5-base-v2~\cite{wang2022text}} & 49.64	&64.19	&66.6	&53.15	&54.45	&31.39	&35.3\\
            % & \multicolumn{2}{l}{CodeT5+~\cite{wang2023codet5opencodelarge}} & 34.67 & 56.93 & 67.15 & 50.73 & 58.39 & 25.55 & 32.85\\
            & \multicolumn{2}{l}{Jina-Code-v2~\cite{günther2023jinaembeddingsnovelset}} & 43.43	&59.93	&63.7	&51.02	&54.13	&33.28	&36.44\\
            & \multicolumn{2}{l}{Codesage-large-v2~\cite{zhang2024code}}  & 47.81	&60.82	&64.39	&49.38	&52.22	&27.03	&30.74\\
            & \multicolumn{2}{l}{CodeRankEmbed~\cite{suresh2024cornstack}} & 52.55	&67.54	&70.39	&57.51	&59.76	&40.28	&42.55\\
        \midrule
        \multirow{2}{*}{Procedure-Based} 
            & \multirow{2}{*}{\makecell[l]{Agentless\\\cite{xia2024agentless}}}  
                & \texttt{GPT-4o}   & 67.15	&71.76	&71.76	&64.31	&64.31	&53.81	&53.81 \\
            & & \texttt{Claude-3.5} & 72.63	&76.72	&76.87	&67.36	&67.36	&57.55	&57.55 \\
        \midrule
        \multirow{9}{*}{Agent-Based} 
            & \multirow{2}{*}{\makecell[l]{MoatlessTools\\\cite{orwall2023moatless}}} 
                & \texttt{GPT-4o}   & 73.36	&80.03	&80.33	&68.57	&69.09	&49.77	&50.62  \\
            & & \texttt{Claude-3.5} & 72.63	&80.73	&80.88	&69.11	&69.11	&53.03	&53.16  \\
        \cmidrule(lr){2-10}ndcg
            & \multirow{2}{*}{\makecell[l]{SWE-agent\\\cite{yang2024sweagent}}}
                & \texttt{GPT-4o}   & 57.3	&63.96	&64.12	&53.95	&53.95	&42.32	&42.44 \\
            &                      & \texttt{Claude-3.5} & 77.37	&84.32	&84.93	&72.77	&72.9	&59.67	&59.79 \\
        \cmidrule(lr){2-10}
            & \multirow{2}{*}{\makecell[l]{Openhands\\\cite{wang2024openhands}}} 
                & \texttt{GPT-4o}   & 60.95	&67.62	&68.39	&58.18	&58.6	&44.34	&44.66  \\
            & & \cellcolor{gray!10}\texttt{Claude-3.5} & 76.28	&84.27	&84.43	&75.79	&75.92	&63.13	&63.8  \\
        \cmidrule(lr){2-10}
            & \multirow{3}{*}{LocAgent (Ours)}
                % & \texttt{GPT-4o}      &63.14	&84.31	&85.77	&74.45	&77.37	&59.85	&65.33  \\
            & \texttt{Qwen2.5-7B(ft)}      & 70.80 & 79.36 & 80.9 & 70.99 & 71.68 & 55.62 & 58.09  \\
            & & \cellcolor{blue!10}\texttt{Qwen2.5-32B(ft)} & \cellcolor{blue!10}75.91 & \cellcolor{blue!10}84.74 & \cellcolor{blue!10}85.64 & \cellcolor{blue!10}76.28 & \cellcolor{blue!10}76.77 & \cellcolor{blue!10}64.27 & \cellcolor{blue!10}65.93  \\
            & & \cellcolor{blue!20}\texttt{Claude-3.5}   & \cellcolor{blue!20}\textbf{77.74} & \cellcolor{blue!20}\textbf{86.19} & \cellcolor{blue!20}\textbf{87.14} & \cellcolor{blue!20}\textbf{77.73} & 
            \cellcolor{blue!20}\textbf{78.1} & 
            \cellcolor{blue!20}\textbf{64.34} & \cellcolor{blue!20}\textbf{65.57} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Precision analysis of different localization methods at various granularities.}
    \label{tab:precision_comparison}
\end{table*}

==> data/main_results.tex <==
\begin{table*}[ht]
\centering
\label{tab:loc_results_lite}
\resizebox{\textwidth}{!}{
\begin{tabular}{cl ccc ccc ccc ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{LM}} & \multicolumn{3}{c}{\textbf{Top-1 file}} & \multicolumn{3}{c}{\textbf{Top-3 file}} & \multicolumn{3}{c}{\textbf{Top-5 file}} & \multirow{2}{*}{\textbf{Avg Tokens}} & \multirow{2}{*}{\textbf{Cost(\$)}} & \multirow{2}{*}{\textbf{\#Convs}} \\ 
\cmidrule{3-11}
 && \textbf{file(\%)} & \textbf{module(\%)} & \textbf{function(\%)} & \textbf{file(\%)} & \textbf{module(\%)} & \textbf{function(\%)} & \textbf{file(\%)} & \textbf{module(\%)} & \textbf{function(\%)} &&& \\ 
 \midrule
 \midrule
\multirow{2}{*}{Agentless} & \texttt{GPT-4o} & 63.3 & 55.0 & 45.3 & 77.0 & 64.9 & 52.9 & 83.0 & 64.9 & 52.9 & 10,909 & 0.0002 & 6\\
 & \texttt{Claude-3.5} & 65.7 & 56.0 & 48.0 & 83.7 & 66.0 & 56.3 & 88.0 & 67.7 & 58.0 & 17,578 & 0.0002 & 6\\ \midrule
 \multirow{2}{*}{Openhands} & \texttt{GPT-4o} & 61.0 & 52.7 & 42.3 & 71.3 & 61.0 & 48.7 & 73.0 & 61.3 & 49.0 &-& 1.560 & 29\\
 & \texttt{Claude-3.5} & 75.7 & \textbf{71.3} & \textbf{62.7} & 89.3 & \textbf{82.3} & 69.7 & 89.7 & \textbf{82.7} & 69.7 & - & 1.456 & 25\\ \midrule
\multirow{2}{*}{moatless} & \texttt{GPT-4o} & 73.3 & 64.3 & 51.0 & 84.0 & 73.7 & 57.3 & 84.7 & 73.7 & 57.3 & - & 0.055\textcolor{gray}{+0.4}& 10 \\
 & \texttt{Claude-3.5} & 72.0 & 63.3 & 56.0 & 85.3 & 73.7 & 64.0 & 85.7 & 74.0 & 64.0 & - & 0.055\textcolor{gray}{+0.4}& 10\\ \midrule
 \multirow{5}{*}{Ours} & \texttt{GPT-4o} & 66.3 & 59.7 & 50.0 & 77.7 & 67.7 & 54.7 & 78.0 & 68.0 & 55.0 &&&\\
 & \texttt{Claude-3.5} & 76.0 & 69.3 & \textbf{62.7} & 89.7 & 80.0 & \textbf{70.0} & \textbf{91.7} & 81.3 & \textbf{70.3} &  105,082 & 0.331 & 14 \\ 
 
   & \texttt{Qwen-Coder-7B} & 43.7 & 33.0 & 20.3 & 56.0 & 41.7 & 24.3 & 56.7 & 41.7 & 24.3 &   &  &  \\ 
 & \texttt{Qwen-Coder-7B(ft)} & 70.3 & 64.3 & 57.0 & 84.3 & 75.3 & 65.7 & 85.0 & 75.7 &67.7 &  81,729 & 0.015 & 12 \\ 

 & \texttt{Qwen-Coder-32B} & 65.7 & 56.0 & 44.0 & 77.7 & 62.7 & 48.0 & 79.0 & 63.3 & 48.3 &   &  &  \\ 
 & \texttt{Qwen-Coder-32B(ft)} & \textbf{76.3} & 71.0 & 61.7 & \textbf{90.0} & 80.7 & 69.3 & 90.7 & 81.0 & 69.7 &  225,361 & 0.041 & 19 \\ 
 \bottomrule
\end{tabular}
}
\caption{File, Module, and Function-Level Localization Recall and Performance and Cost Analysis}
% \vspace{-5mm}
\end{table*}

==> data/time_efficiency.tex <==
% \begin{table}[ht!]
%     \centering
%     \small
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{lcccc}
%         \toprule
%         % Method & Index Time (s) & Retrieval Time (s) & Total Time (s) \\
%         % \midrule
%         % BM25 & - & - & - \\
%         % CodeSage-Large & - & - & - \\
%         % CodeT5+ & - & - & - \\
%         % Jina-Code-v2 & - & - & - \\
%         % CodeRankEmbed & - & - & - \\
%         \textbf{Method} & \textbf{Param.} & \textbf{Index Time (s)} & \textbf{Retrieval Time (s)} & \textbf{Memory Footprint (GB)} \\
%         \midrule
%         BM25 & - & - & - & - \\
%         e5-base & 110M & 34 & 5.4 & 4 \\
%         e5-base-v2 & 110M & 34 & 5.4 & 4 \\
%         CodeSage-Large & 1.3B & 34 & 81 & 41 \\
%         Codesage-large-v2 & 1.3B & 34 & 83 & 41 \\
%         CodeT5+ & 110M & 34 & 23.5 & 13 \\
%         Jina-Code-v2 & 161M & 34 & 13 & 28 \\
%         CodeRankEmbed & 137M & 34 & 15 & 24 \\
%         % SFR-Embedding-Mistral & 7B & 34 & 138 & 77 \\
%         \midrule
%         Agentless & - & - & - \\
%         openhands & - & - & - \\
%         moatless & - & - & - \\
%         Ours & - & - & - \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Computational efficiency comparison of different code indexing methods.}
%     \label{tab:time_efficiency}
% \end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllrr}
\toprule
\textbf{Method}          & \textbf{Device} & \textbf{Parallelism} & \makecell[c]{\textbf{Latency} \\ \textbf{per repo}} & \textbf{Total time} \\ \midrule \midrule
\textsc{LocAgent}                & CPU             & repo-level           & 587s                           & 0.9h                     \\ 
E5-base-v2              & GPU             & chunk-level          & 45s                            & 1.2h                     \\ 
Jina-Code-v2            & GPU             & chunk-level          & 53s                            & 1.8h                     \\ 
Codesage-large-v2       & GPU             & chunk-level          & 123s                           & 7h                       \\ 
CodeRankEmbed           & GPU             & chunk-level          & 55s                            & 1.9h                     \\ \bottomrule
\end{tabular}
}
\caption{Time efficiency comparison of different code indexing methods.}
\label{tab:time_efficiency}
\end{table}

